Fixed-point iterations for several dissimilarity measure barycenters in the Gaussian case

In target tracking and sensor fusion contexts it is not unusual to deal with a large number of Gaussian densities that encode the available information (multiple hypotheses), as in applications where many sensors, affected by clutter or multimodal noise, take measurements on the same scene. In such cases reduction procedures must be implemented, with the purpose of limiting the computational load. In some situations it is required to fuse all available information into a single hypothesis, and this is usually done by computing the barycenter of the set. However, such computation strongly depends on the chosen dissimilarity measure, and most often it must be performed making use of numerical methods, since in very few cases the barycenter can be computed analytically. Some issues, like the constraint on the covariance, that must be symmetric and positive definite, make it hard the numerical computation of the barycenter of a set of Gaussians. In this work, Fixed-Point Iterations (FPI) are presented for the computation of barycenters according to several dissimilarity measures, making up a useful toolbox for fusion/reduction of Gaussian sets in applications where specific dissimilarity measures are required.

==> titles.tex <==
\title{
\large Some title proposals:\\[10pt]
\Large \bf Fixed-point recursions for several dissimilarity measure barycenters \\
in the Gaussian case\\[12pt]
Fixed-point recursive computation of barycenters \\
for several dissimilarity measure in the Gaussian case\\[12pt]
Barycenter computation for several dissimilarity measures \\
by means of Fixed-point recursions: the Gaussian case\\[12pt]
Sets of Gaussians barycenter computation for several dissimilarity measures \\
by means of fixed point recursions\\[12pt]
Fixed-point iterative computation of barycenters of sets of Gaussians \\ 
for several dissimilarity measures
}

